Semantic Scene Completion via Integrating Instances and Scene in-the-Loop

Semantic Scene Completion aims at reconstructing a complete 3D scene with precise voxel-wise semantics from a single-view depth or RGBD image. It is a crucial but challenging problem for indoor scene understanding. In this work, we present a novel framework named Scene-Instance-Scene Network (\textit{SISNet}), which takes advantages of both instance and scene level semantic information. Our method is capable of inferring fine-grained shape details as well as nearby objects whose semantic categories are easily mixed-up. The key insight is that we decouple the instances from a coarsely completed semantic scene instead of a raw input image to guide the reconstruction of instances and the overall scene. SISNet conducts iterative scene-to-instance (SI) and instance-to-scene (IS) semantic completion. Specifically, the SI is able to encode objects' surrounding context for effectively decoupling instances from the scene and each instance could be voxelized into higher resolution to capture finer details. With IS, fine-grained instance information can be integrated back into the 3D scene and thus leads to more accurate semantic scene completion. Utilizing such an iterative mechanism, the scene and instance completion benefits each other to achieve higher completion accuracy. Extensively experiments show that our proposed method consistently outperforms state-of-the-art methods on both real NYU, NYUCAD and synthetic SUNCG-RGBD datasets. The code and the supplementary material will be available at \url{https://github.com/yjcaimeow/SISNet}.

==> semantic scene completion/tables/GRNet.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[t!]
% \small
% \begin{center}
% %\vspace{-4.5cm}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|cccc|}
% \hline
%                                             & Layer name     & Input                           & Output size    \\ \hline                & Layer params                  \\ \hline
                                            
% \multirow{3}{*}{Semantic Encoder}           & FC\_1          & Semantic Vector                  & (16, 1)         \\   %              & (8,16)                        \\
%                                             & FC\_2          & FC\_1                           & (64, 1)           \\  %            & (16,64)                       \\
%                                             & Reshape\_1     & FC\_2                           & (1, $4^{3}$)    \\\hline%   &  -                             \\ \hline
% \multirow{6}{*}{Geometry Encoder}           & Griding        & Partial Point Cloud             & (1, $32^{3}$)   \\%   &   -                            \\
%                                             & Conv3D\_1      & 3D Grid                         & (16, $16^{3}$)  \\%  & (16, $4^{3}$) \\
%                                             & Conv3D\_2      & Conv3D\_1                       & (32, $8^{3}$)   \\%  & (32, $4^{3}$) \\
%                                             & Conv3D\_3      & Conv3D\_2                       & (32, $4^{3}$)   \\%  & (32, $4^{3}$) \\ 

%                                             & Concat\_1      & Conv3D\_3, Reshape\_1                 & (33, $4^{3}$) \\% &  -                             \\
%                                             & Conv3D\_4      & Concat\_1                       & (32, $4^{3}$)  & \\ \hline  %(1, $1^{3}$)  \\ \hline 
%  \multirow{3}{*}{Decoder}                                             & Deconv3D\_1    & Conv3D\_4             & (32, $8^{3}$)  \\ %& (32, $4^{3}$) \\
%                                             & Deconv3D\_2    & Concat(Deconv3D\_1, Conv3D\_2)          & (16, $16^{3}$) \\ %& (16, $4^{3}$) \\
%                                             & Deconv3D\_3    & Concat(Deconv3D\_2, Conv3D\_1)          & (1, $32^{3}$)  \\ \hline%& (1, $4^{3}$)  \\ \hline
% \multirow{5}{*}{Feature-Point 
%                 downsampling(ds)}               & Re-Griding     & Deconv3D\_1                     & (1, $32^{3}$)      \\  %       &   -       \\
%                                             & Point\_ds      & Re-Griding, Partical Point Cloud & (3, 1024)              \\  %        &   -                            \\
%                                             & Feature\_ds\_1 & ConCat(Point\_ds, Conv3D\_2)             & (128, 1024)     \\ %               &   -                            \\ %\cline{2-5} 
%                                             & Feature\_ds\_2 & ConCat(Point\_ds, Conv3D\_1)            & (256, 1024)      \\  %              &   -                            \\
%                                             & Concat\_2      & Feature\_DS\_1, Feature\_DS\_2     & (384, 1024)            \\ \hline %       &   -                            \\ \hline
% \multirow{4}{*}{MLP}                        & FC\_3          & Concat\_2                       & (96, 1024)                \\ %     & (384, 96)                      \\
%                                             & FC\_4          & FC\_3                           & (24, 1024)               \\ %      & (96, 24)                       \\
%                                             %& Tile\_1        & Point\_ds)                      & (3, 8192)                       &   -                   \\ %\hline
%                                             & Reshape\_2     & FC\_4                           & (3, 8192)                \\ %       &   -                           \\ %\hline
%                                             & Output         & Tile(Point\_ds)+Reshape\_2      & (3, 8192)                \\ \hline      &   -                           \\ \hline
% \end{tabular}
% }

% \end{center}
% %\vsapce{0.2cm}
% \caption{Parameter details of shape reconstruction module.Tile means a operation that replicate the input $(3,m)$ $n$ times and return a new point set with the size of $(3,mn)$.}
% \label{tab:arch_grnet}
% \end{table*}
%\multirow{2}{*}{}  

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
                                                                                       & Layer name     & Input                           & Output size                    \\ \hline
\multirow{3}{*}{Semantic Encoder}                                                      & FC\_1          & Semantic Vector                 & (16,1)                         \\
                                                                                       & FC\_2          & FC\_1                           & (64,1)                         \\
                                                                                       & Reshape\_1     & FC\_2                           & (1, $4^{3}$)   \\ \hline
\multirow{6}{*}{Geometry Encoder}                                                      & Griding        & Partial Point Cloud             & (1, $32^{3}$) \\
                                                                                       & Conv3D\_1      & Griding                         & (16, $16^{3}$)                      \\
                                                                                       & Conv3D\_2      & Conv3D\_1                       & (32, $8^{3}$)                     \\
                                                                                       & Conv3D\_3      & Conv3D\_2                       & (32, $4^{3}$)                     \\
                                                                                       & Concat\_1      & Conv3D\_3, FC\_2                 & (33, $4^{3}$)  \\
                                                                                       & Conv3D\_4      & Concat\_1                       & (32, $4^{3}$)  \\ \hline
\multirow{3}{*}{Decoder}                                                               & Deconv3D\_1    & Conv3D\_4                       & (32, $8^{3}$) \\
                                                                                       & Deconv3D\_2    & Deconv3D\_1, Conv3D\_2           & (32, $16^{3}$) \\
                                                                                       & Deconv3D\_3    & Deconv3D\_2, Conv3D\_1           & (32, $32^{3}$)  \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Feature-Point\\  DownSampling(DS)\end{tabular}} & Rev-Griding     & Deconv3D\_3                     & (1, $32^{3}$)   \\
                                                                                       & Point\_DS      & Rev-Griding, Partial Point Cloud & (3,1024)                       \\
                                                                                       & Feature\_DS\_1 & Point\_DS, Conv3D\_2             & (128,1024)                     \\ %\cline{2-4} 
                                                                                       & Feature\_DS\_2 & Point\_DS, Conv3D\_1             & (256,1024)                     \\
                                                                                       & Concat\_2      & Feature\_DS\_1, Feature\_DS\_2   & (384,1024)                     \\ \hline
\multirow{4}{*}{MLP}                                                                   & FC\_3          & Concat\_2                       & (96,1024)                      \\
                                                                                       & FC\_4          & FC\_3                           & (24,1024)                      \\
                                                                                       & Reshape\_2     & FC\_4                           & (3,8192)                       \\ %\hline
                                                                                       & Output         & Tile(Point\_DS), Reshape\_2      & (3, 8192)                \\ \hline 
\end{tabular}
}
\vspace{0.2cm}
\caption{Architecture details of shape completion. Tile denotes a operation that replicate the input $(3,m)$ $n$ times and return a new point set with the size of $(3,m\times n)$. We use the Griding, Rev-Griding and downsampling operations proposed in \cite{xie2020grnet}}
\label{tab:arch_grnet}
\end{table}

==> semantic scene completion/tables/Scene.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[t!]
% % \vspace{-1.0cm}
% \begin{center}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|ccccc|}
% \hline
%                           & Layer name   & Input                                     & Type & Output size    & Layer params                       \\ \hline
% \multirow{14}{*}{Encoder} & Conv3D\_1\_0 & Semantic Volume $V_S$                        & CBR  & (3,  60,  36,  60)   & (1,  3,  3\textasciicircum{}\{3\})     \\
%                           & Conv3D\_1\_1 & Conv3D\_1\_0                              & CBR  & (64,  60,  36,  60)  & (3,  64,  3\textasciicircum{}\{3\})    \\
%                           & Conv3D\_1\_2 & Conv3D\_1\_1                              & CBR  & (128,  60,  36,  60) & (64,  128,  3\textasciicircum{}\{3\})  \\
%                           & Conv3D\_2\_0 & TSDF Volume $V_T$                            & CBR  & (3,  60,  36,  60)   & \color{red}{(12,  3,  3\textasciicircum{}\{3\})}    \\
%                           & Conv3D\_2\_1 & Conv3D\_2\_0                              & CBR  & (64,  60,  36,  60)  & (3,  64,  3\textasciicircum{}\{3\})    \\
%                           & Conv3D\_2\_2 & Conv3D\_2\_1                              & CBR  & (128,  60,  36,  60) & (64,  128,  3\textasciicircum{}\{3\})  \\ \cline{2-6} 
%                           & DDR\_0       & Conv3D\_1\_2+Conv3D\_2\_2                 & DDR  & (128,  30,  18,  30) & (1,  2)                              \\
%                           & DDR\_1\_1    & DDR\_0                                    & DDR  & (128,  30,  18,  30) & (1,  1)                              \\
%                           & DDR\_1\_2    & DDR\_1\_1                                 & DDR  & (128,  30,  18,  30) & (2,  1)                              \\
%                           & DDR\_1\_3    & DDR\_1\_2                                 & DDR  & (128,  30,  18,  30) & (3,  1)                              \\ \cline{2-6} 
%                           & DDR\_2       & DDR\_1\_3+Down & DDR  & (256,  15,  9,  15)  & (1,  2)                              \\
%                           & DDR\_3\_1    & DDR\_2                                    & DDR  & (256,  15,  9,  15)  & (1,  1)                              \\
%                           & DDR\_3\_2    & DDR\_3\_1                                 & DDR  & (256,  15,  9,  15)  & (2,  1)                              \\
%                           & DDR\_3\_3    & DDR\_3\_2                                 & DDR  & (256,  15,  9,  15)  & (3,  1)                              \\ \hline
% \multirow{3}{*}{Decoder}  & Deconv3D\_1  & DDR\_3\_3 + DDR\_1\_3 + Down              & CBR  & (128,  30,  18,  30) & (256,  128,  3\textasciicircum{}\{3\}) \\
%                           & Deconv3D\_2  & Deconv3D\_1                               & CBR  & (128,  60,  36,  60) & (128,  128,  3\textasciicircum{}\{3\}) \\
%                           & Conv3D\_3    & Deconv3D\_2 + Up                              & Conv     & (12,  60,  36,  60)  & (128,  12,  1\textasciicircum{}\{3\})  \\ \hline
% \end{tabular}
% }
% \end{center}
% \caption{Architecture and parameters details of scene completion stage. $Down$ means the downsampling operation of the combination feature of (Conv3D\_1\_2+Conv3D\_2\_2) while the $Up$ is the upsampling operation on output feature of Deconv3D\_1.CBR denotes a convolution block consists of a convolution layer flowed by a batchnorm layer and Relu function while Conv means a single a convolution layer.For DDR block, the layer params represents the dilation and downsample rate, respectively.}
% \label{tab:arch_scene}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
\small
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|}
\hline
                                                                             & Layer name   & Input                     & Type & Output size    \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Semantic\\ Encoder\end{tabular}}  & Conv3D\_1\_0 & Semantic Volume V_S        & CBR  & (3,60,36,60)   \\
                                                                             & Conv3D\_1\_1 & Conv3D\_1\_0              & CBR  & (64,60,36,60)  \\
                                                                             & Conv3D\_1\_2 & Conv3D\_1\_1              & CBR  & (128,60,36,60) \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Geometry \\ Encoder\end{tabular}} & Conv3D\_2\_0 & TSDF Volume V_T            & CBR  & (3,60,36,60)   \\
                                                                             & Conv3D\_2\_1 & Conv3D\_2\_0              & CBR  & (64,60,36,60)  \\
                                                                             & Conv3D\_2\_2 & Conv3D\_2\_1              & CBR  & (128,60,36,60) \\
                                                                             & Add\_1       & Conv3D\_1\_2, Conv3D\_2\_2 & -     & (128,60,36,60) \\ \hline
\multirow{9}{*}{Encoder}                                                     & DDR\_0       & Add\_1                       & DDR  & (128,30,18,30) \\
                                                                             & DDR\_1       & DDR\_0                    & DDR  & (128,30,18,30) \\
                                                                             & DDR\_2       & DDR\_1                    & DDR  & (128,30,18,30) \\
                                                                             & DDR\_3       & DDR\_2                    & DDR  & (128,30,18,30) \\
                                                                             & Add\_2       & DDR\_3, Down(Add\_1)       & -    & (128,30,18,30) \\ \cline{2-5} 
                                                                             & DDR\_4       & Add\_2                    & DDR  & (256,15,9,15)  \\
                                                                             & DDR\_5       & DDR\_4                    & DDR  & (256,15,9,15)  \\
                                                                             & DDR\_6       & DDR\_5                    & DDR  & (256,15,9,15)  \\
                                                                             & DDR\_7       & DDR\_6                    & DDR  & (256,15,9,15)  \\ \hline
\multirow{4}{*}{Decoder}                                                     & Deconv3D\_1  & DDR\_7                    & DBR  & (128,30,18,30) \\
                                                                             & Add\_3       & Deconv3D\_1, Add\_2        & -    & (128,30,18,30) \\
                                                                             & Deconv3D\_2  & Add\_3                    & DBR  & (128,60,36,60) \\
                                                                             & Conv3D\_3    & Deconv3D\_2, Up(Add\_3)    & Conv & (12,60,36,60)  \\ \hline
\end{tabular}
}
\end{center}
\caption{Architecture and parameters details of scene completion stage. \textit{Down}, \textit{Up} mean downsampling and upsampling operation, respectively. \textit{CBR} denotes a convolution block consists of a $3\times 3$ convolution layer flowed by a batchnorm layer and Relu function and \textit{DBR} replaces the convolution layer of \textit{CBR} with a $4\times 4$ deconvolution layer.  \textit{Conv} means a single  $1\times 1$ convolution layer.}
\label{tab:arch_scene}
\end{table}

==> semantic scene completion/tables/ablation-cost.tex <==
\begin{table}[t]
\begin{center}
\resizebox{0.85\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
\textbf{Method} & \textbf{SC(\%)} & \textbf{SSC(\%)} &\textbf{Params/M}\\
\hline
Sketch~\cite{Chen_2020_SketchAwareSSC} & 71.3 & 41.1  &28.0\\
Ours (BiSeNet)   &77.8& 49.8 & 30.5\\
Ours (DeepLabv3)   &78.2& 52.4 & 47.3\\
\hline
\end{tabular}
}

\end{center}
\vspace{-0.2cm}
\caption{Efficiency with different methods on NYU dataset.}
\label{tab:ablation-cost}
\vspace{-0.3cm}
\end{table}
%\vspace{-0.3cm}

==> semantic scene completion/tables/ablation-detection.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t!]
\tiny
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|ccccccccc|c|}
\hline
Datasets                    & Iteration       & win.          & chair         & bed           & sofa          & table         & tvs           & furn.         & objs.         & avg           \\ \hline
\multirow{3}{*}{NYU}        & I               & 7.5           & 21.1          & 59.6          & 45.7          & 20.1          & 18.0          & 27.6          & 7.4           & 25.6          \\
                            & S0 + Iter I-S   & 15.8          & 30.0          & 66.0          & 48.8          & 29.8          & 31.6          & 35.9          & 19.0          & 34.6          \\
                            & S0 + 2 Iter I-S & \textbf{21.9} & \textbf{33.2} & \textbf{69.0} & \textbf{55.8} & \textbf{43.4} & \textbf{36.3} & \textbf{43.2} & \textbf{23.8} & \textbf{40.8} \\ \hline
\multirow{3}{*}{NYUCAD}     & I               & 32.7          & 38.3          & 64.9          & 54.4          & 43.1          & 35.1          & 38.9          & 21.7          & 41.1          \\
                            & S0 + Iter I-S   & 30.1          & 50.0          & 66.6          & 52.3          & 44.0          & 36.8          & 46.3          & 31.3          & 44.5          \\
                            & S0 + 2 Iter I-S & \textbf{42.0} & \textbf{50.2} & \textbf{72.3} & \textbf{60.5} & \textbf{58.5} & \textbf{46.7} & \textbf{54.3} & \textbf{37.2} & \textbf{52.7} \\ \hline
\multirow{3}{*}{SUNCG-RGBD} & I               & 74.2          & 65.0          & 83.9          & 82.0          & 67.3          & 32.7          & 72.1          & 43.3          & 65.0          \\
                            & S0 + Iter I-S   & 76.1          & 75.7          & 85.2          & \textbf{84.2} & 70.8          & \textbf{35.6} & 82.6          & 53.3          & 70.4          \\
                            & S0 + 2 Iter I-S & \textbf{76.8} & \textbf{76.9} & \textbf{86.6} & 83.2          & \textbf{72.9} & 34.0          & \textbf{86.0} & \textbf{56.5} & \textbf{71.6} \\ \hline
\end{tabular}
}
\end{center}
\caption{Ablation studies of the effects of the scene completion to the proposal generation module of instance completion on three datasets. The numbers reported are detection mAP (IoU=0.25) for different classes, where $I$ is the instance completion and $S$ is the scene completion.}
\label{tab:detection}
\end{table*}

==> semantic scene completion/tables/ablation-instance.tex <==
\begin{table}[t]
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|} 
\hline
\textbf{Scheme} & \textbf{Dataset} & \textbf{SC-IoU(\%)} & \textbf{SSC-mIoU(\%)} \\

%\hline
%Baseline &  NYU  & 70.8 & 45.6\\
%+ Scene &  NYU & -- & -- \\
%+ Instance &  NYU  & \textbf{78.2} & \textbf{52.4}\\
%\hline
%Baseline &  NYUCAD  & 82.8 & 57.4\\
%+ Scene &  NYUCAD & 83.7 & 58.3 \\
%+ Instance &  NYUCAD  & \textbf{86.3} & \textbf{63.5}\\
%\hline
%Baseline &  SUNCG  & 85.6 & 72.9\\
%+ Scene &  SUNCG & -- & -- \\
%+ Instance &  SUNCG  & \textbf{--} & \textbf{--}\\
%\hline
\hline
Baseline ($S_0$) &  NYU  & 71.0 & 42.5\\
\textit{+$S_1$ only} &  NYU & 75.4 \textcolor{blue}{(+4.4)}& 44.9 \textcolor{blue}{(+2.4)}\\
\textit{+Iter I-S} &  NYU  & 76.4 \textcolor{blue}{(+5.4)} & 47.7 \textcolor{blue}{(+5.2)}\\
+\textit{2-Iter I-S} & NYU &\textbf{77.8 \textcolor{blue}{(+6.8)}}&\textbf{49.8 \textcolor{blue}{(+7.3)}}\\
\hline
Baseline ($S_0$) &  NYUCAD  & 82.8 & 53.6\\
\textit{+$S_1$ only} &  NYUCAD & 83.3 \textcolor{blue}{(+0.5)}& 54.2 \textcolor{blue}{(+0.6)}\\
\textit{+Iter I-S} &  NYUCAD & 85.1 \textcolor{blue}{(+2.3)}& 58.0 \textcolor{blue}{ (+4.4)}\\
+\textit{2-Iter I-S} & NYUCAD & \textbf{86.5 \textcolor{blue}{(+3.7)}}&\textbf{59.9 \textcolor{blue}{(+6.3)}}\\
\hline
Baseline ($S_0$) &  SUNCG-RGBD  & 86.0 & 73.0\\
\textit{+$S_1$ only} &  SUNCG-RGBD & 87.8 \textcolor{blue}{(+1.8)}& 74.5 \textcolor{blue}{(+1.5)} \\
\textit{+Iter I-S} &  SUNCG-RGBD  & 88.4 \textcolor{blue}{(+2.4)} & 76.6 \textcolor{blue}{(+3.6)}\\
+\textit{2-Iter I-S} & SUNCG-RGBD & \textbf{89.9 \textcolor{blue}{(+3.9)}}&\textbf{78.8 \textcolor{blue}{(+5.8)}}\\
\hline
\end{tabular}
}
% \vspace{-0.6cm}
\end{center}
\vspace{-0.2cm}
\caption{Ablation studies of the effects of \textbf{instance completion}.}
\label{tab:ablation-instance}
\vspace{-0.3cm}
\end{table}
%\vspace{-0.3cm}

==> semantic scene completion/tables/ablation-iteration.tex <==
\begin{table*}[t!]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|c |c c c|c c c c c c c c c c c | c|} 
\hline
%   & \multicolumn{3}{c|}{scene completion} & \multicolumn{12}{c}{semantic scene completion} \\ \hline
% Methods  & prec. & recall & IoU & \cellcolor{rgb1}ceil. & \cellcolor{rgb2}floor & \cellcolor{rgb3}wall & \cellcolor{rgb4}win. & \cellcolor{rgb5}chair & \cellcolor{rgb6}bed & \cellcolor{rgb7}sofa & \cellcolor{rgb8}table & \cellcolor{rgb9}tvs & \cellcolor{rgb10}furn. & \cellcolor{rgb11}objs. & avg. \\ 
  & & \multicolumn{3}{c|}{Scene Completion (SC)} & \multicolumn{12}{c|}{Semantic Scene Completion (SSC)} \\ \hline
Methods & Trained on & prec. & recall & IoU & ceil. & floor & wall & win. & chair & bed & sofa & table & tvs & furn. & objs. & avg. \\ 
\hline
Baseline & NYU  &	87.6&	78.9& 71.0&46.9&	93.3&	41.3&	26.7&	30.8&	58.4&	49.5&	27.2&	22.1&	42.2&	28.7&	42.5\\
+\textit{Iter I-S} & NYU  &	91.1&	82.5&76.4&	52.5&	93.6&	50.7&	35.4&	37.3&	62.8&	54.1&	34.0&	22.2&	48.7&	33.8&	47.7\\
+\textit{2-Iter I-S} & NYU  &90.7&	84.6&	77.8& 53.9&	93.2&	51.3&	38.0&	38.7&	65.0&	56.3&	37.8&	25.9&	51.3&	36.0&	49.8\\ 
\hline
Baseline  & NYUCAD  &	
92.3&	89.0&	82.8&	61.5&	94.2&	62.7&	38.0&	48.1&	69.5&	59.3&	40.1&	25.8&	54.6&	35.3&	53.6\\
+\textit{Iter I-S}  & NYUCAD  &	
93.4&	90.5&	85.1&	63.8&	94.4&	65.1&	43.0&	54.1&	73.9&	64.7&	47.8&	30.4&	60.2&	40.6&	58.0\\
+\textit{2-Iter I-S}& NYUCAD  &	
94.2&	91.3&	86.5&	65.6&	94.4&	67.1&	45.2&	57.2&	75.5&	66.4&	50.9&	31.1&	62.5&	42.9&	59.9\\
\hline

Baseline& SUNCG-RGBD  &	
90.6&	94.5&	86.0&	71.0&	86.6&	78.4&	78.7&	53.2&	77.4&	77.3&	60.6&	76.4&	83.7&	60.0&	73.0\\
+\textit{Iter I-S} & SUNCG-RGBD  &
92.2&	95.5&	88.4&	79.3&	88.8&	82.5&	80.4&	56.8&	81.2&	79.5&	63.8&	77.9&	85.3&	67.1&	76.6\\
+\textit{2-Iter I-S }  & SUNCG-RGBD  &
93.3&	96.1&	89.9&	85.2&	90.0&	83.7&	80.8&	60.0&	83.5&	80.9&	68.6&	77.3&	86.7&	70.1&	78.8\\
\hline
\end{tabular}
}
% \vspace{-0.6cm}
\end{center}
\vspace{-0.2cm}
\caption{Ablation studies of the effects of \textbf{scene-instance-scene iterations} on NYU, NYUCAD and SUNCG-RGBD dataset.}
\label{tab:ablation-iteration}
\vspace{-0.3cm}
\end{table*}

==> semantic scene completion/tables/ablation-order.tex <==
\begin{table}[t]
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
\textbf{Order} & \textbf{Dataset} &\textbf{Rec.} &\textbf{mAP}
&\textbf{Shape} & \textbf{SC} & \textbf{SSC} \\
\hline
Baseline ($S_0$) &  NYU  &-&-& -& 71.0 & 42.5\\
\textit{$I_1$-$S_1$}  &  NYU   &61.7& 25.9 & 25.9 & 75.5& 46.6\\
\textit{$S_0$-$I_1$-$S_1$} &  NYU &\textbf{68.8}&\textbf{34.6} &\textbf{35.1}&\textbf{76.4} & \textbf{47.7}\\
\hline
% use C1_W3
Baseline ($S_0$) &  NYUCAD  &-&- &-&82.8 & 53.6\\
\textit{$I_{1}$-$S_{1}$} &  NYUCAD &75.0 &41.1 &30.1  & 83.1& 55.5\\
\textit{$S_0$-$I_{1}$-$S_{1}$} &  NYUCAD &\textbf{76.8} &\textbf{44.5}& \textbf{43.3} & \textbf{85.1}& \textbf{58.0}\\
\hline
Baseline ($S_{0}$) &  SUNCG-RGBD  &-&-&-& 86.0 & 73.0\\
\textit{$I_{1}$-$S_{1}$} &  SUNCG-RGBD &77.6 &65.0 &41.7 & 87.5 &75.8\\
\textit{$S_{0}$-$I_{1}$-$S_{1}$} &  SUNCG-RGBD&\textbf{81.2} &\textbf{70.4} &\textbf{50.1}  &\textbf{88.4}& \textbf{76.6}\\
\hline
\end{tabular}
}
% \vspace{-0.6cm}
\end{center}
\vspace{-0.2cm}
\caption{Ablation studies of effects of \textbf{initial scene completion}, where Rec. (recall) and mAP (IoU=0.25) denote the instance detection performance. Shape means the shape completion results.}
\label{tab:ablation-order}
\vspace{-0.6cm}
\end{table}

% \begin{table*}[ht]
% \begin{center}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|l|c |c c|c c c c c c c c c c c | c|} 
% \hline
% %   & \multicolumn{3}{c|}{scene completion} & \multicolumn{12}{c}{semantic scene completion} \\ \hline
% % Methods  & prec. & recall & IoU & \cellcolor{rgb1}ceil. & \cellcolor{rgb2}floor & \cellcolor{rgb3}wall & \cellcolor{rgb4}win. & \cellcolor{rgb5}chair & \cellcolor{rgb6}bed & \cellcolor{rgb7}sofa & \cellcolor{rgb8}table & \cellcolor{rgb9}tvs & \cellcolor{rgb10}furn. & \cellcolor{rgb11}objs. & avg. \\ 
%   & & \multicolumn{2}{c|}{scene completion} & \multicolumn{12}{c|}{semantic scene completion} \\ \hline
% Scheme & Dataset & prec.  & IoU & ceil. & floor & wall & win. & chair & bed & sofa & table & tvs & furn. & objs. & avg. \\ 
% \hline
% Instance-Scene（Detection）  & NYU  &	78.9& 71.0&46.9&	93.3&	41.3&	26.7&	30.8&	58.4&	49.5&	27.2&	22.1&	42.2&	28.7&	42.5\\
% Instance-Scene (ins. shape )& NYU  &	82.5&76.4&	52.5&	93.6&	50.7&	35.4&	37.3&	62.8&	54.1&	34.0&	22.2&	48.7&	33.8&	47.7\\
% Scene-Instance（Detection) & NYU  &	84.6&	77.8& 53.9&	93.2&	51.3&	38.0&	38.7&	65.0&	56.3&	37.8&	25.9&	51.3&	36.0&	49.8\\ 
% Scene-Instance（(ins. shape ) & NYU &	84.6&	77.8& 53.9&	93.2&	51.3&	38.0&	38.7&	65.0&	56.3&	37.8&	25.9&	51.3&	36.0&	49.8\\ 
% \hline
% Instance-Scene（Detection） & NYUCAD  &	89.0&	82.8&	61.5&	94.2&	62.7&	38.0&	48.1&	69.5&	59.3&	40.1&	25.8&	54.6&	35.3&	53.6\\
% Instance-Scene (ins. shape )  & NYUCAD &	90.5&	85.1&	63.8&	94.4&	65.1&	43.0&	54.1&	73.9&	64.7&	47.8&	30.4&	60.2&	40.6&	58.0\\
% Scene-Instance（Detection) & NYUCAD  &	91.3&	86.5&	65.6&	94.4&	67.1&	45.2&	57.2&	75.5&	66.4&	50.9&	31.1&	62.5&	42.9&	59.9\\
% Scene-Instance（(ins. shape ) & NYUCAD  &	84.6&	77.8& 53.9&	93.2&	51.3&	38.0&	38.7&	65.0&	56.3&	37.8&	25.9&	51.3&	36.0&	49.8\\ 
% \hline

% Instance-Scene（Detection） & SUNCG &	89.0&	82.8&	61.5&	94.2&	62.7&	38.0&	48.1&	69.5&	59.3&	40.1&	25.8&	54.6&	35.3&	53.6\\
% Instance-Scene (ins. shape )  & SUNCG &	90.5&	85.1&	63.8&	94.4&	65.1&	43.0&	54.1&	73.9&	64.7&	47.8&	30.4&	60.2&	40.6&	58.0\\
% Scene-Instance（Detection) & SUNCG  &	91.3&	86.5&	65.6&	94.4&	67.1&	45.2&	57.2&	75.5&	66.4&	50.9&	31.1&	62.5&	42.9&	59.9\\
% Scene-Instance（(ins. shape ) & SUNCG &	84.6&	77.8& 53.9&	93.2&	51.3&	38.0&	38.7&	65.0&	56.3&	37.8&	25.9&	51.3&	36.0&	49.8\\ 
% \hline
% \end{tabular}
% }
% % \vspace{-0.6cm}
% \end{center}
% \caption{\textbf{Ablation studies on different orders of instance-reconstruction and scene-refine.}}
% \label{tab:ablation-iteration}
% \end{table*}

==> semantic scene completion/tables/detection_backbone.tex <==
% \begin{table}[t!]
% \small
% \begin{center}
% %\vspace{-1.5cm}
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% Layer & Input                          & Type & Output size  & Layer params                 \\ \hline
% $sa1_0$     & location        & \textit{SA}   & (2048, 3+128) & (2048, 0.2, (64,64,128))   \\
% $sa1_1$     & semantic & \textit{SA}   & (2048, 3+128) & (2048, 0.2, (64,64,128))   \\
% sa2      & $sa1_0$ + $sa1_1$                & \textit{SA}   & (1024, 3+256) & (1024, 0.4, (128,128,256)) \\
% sa3      & sa2                          & \textit{SA}   & (512, 3+256)  & (512, 0.8, (128,128,256))  \\
% sa4      & sa3                          & \textit{SA}   & (256, 3+256)  & (256, 1.2, (128,128,256))  \\
% fp1      & sa3, sa4                        & \textit{FP}   & (512, 3+256)  &(256, 256)               \\
% fp2      & sa2, sa3                        & \textit{FP}   & (1024, 3+256) & (256, 256)              \\ \hline
% offset\_1  & fp\_2                          & \textit{CBR}  & 1024, 256)   & (256, 256, 1                  \\
% offset\_2  & offset\_1                      & \textit{CBR}  & 1024, 256)   & (256, 256, 1)                 \\
% offset\_3  & offset\_2                      & \textit{Conv} & 1024, 3+256) & (256, 256, 1)                  \\ \hline
% proposal\_1       & offset\_3                      & \textit{CBR}  & (256, 128)    & 128, 128, 1                  \\
% proposal\_2       & conv\_1                        & \textit{CBR}  & (256, 128)    & (128, 128, 1)                  \\
% proposal\_3       & conv\_2                        & \textit{Conv} & (256, 62)     & (128, 62, 1)                   \\ \hline
% \end{tabular}
% }
% % \vspace{0.5cm}
% \end{center}
% \caption{Architecture details of proposal generation. \textit{SA} and \textit{FP} represent set abstraction layer and feature propagation layer, respectively. \textit{CBR} denotes a convolution block consists of a convolution layer followed by a batchnorm and Relu function while \textit{Conv} means a single a convolution layer.}
% \label{tab:arch_detection}
% \end{table}

\begin{table}[]
\begin{center}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
Layer name  & Input                          & Type & Output size  \\ \hline
sa\_1\_0      & location of point cloud        & SA   & (2048, 3+128) \\
sa\_1\_1     & semantic vector of point cloud & SA   & (2048, 3+128) \\
sa\_2       & sa\_1\_0, sa\_1\_1             & SA   & (1024,3+256) \\
sa\_3       & sa\_2                          & SA   & (512, 3+256)  \\
sa\_4       & sa\_3                          & SA   & (256, 3+256)  \\
fp\_1       & sa\_3, sa\_4                        & FP   & (512, 3+256)  \\
fp\_2       & sa\_2, sa\_3                        & FP   & (1024, 3+256) \\ \hline
offset\_1   & fp\_2                          & CBR  & （1024, 256)   \\
offset\_2   & offset\_1                      & CBR  & (1024, 256)   \\
offset\_3   & offset\_2                      & Conv & (1024, 3+256) \\ \hline
proposal\_1 & offset\_3                      & CBR  & (256, 128)    \\
proposal\_2 & proposal\_1                        & CBR  & (256, 128）    \\
proposal\_3 & proposal\_2                        & Conv & (256, 62)     \\ \hline
\end{tabular}
}
\end{center}
\caption{Architecture details of proposal generation. \textit{SA} and \textit{FP} represent the set abstraction layer and feature propagation layer, respectively. \textit{CBR} denotes a convolution block consists of a $1\times 1$ convolution layer followed by a batchnorm and Relu function while \textit{Conv} means a single $1\times 1$ convolution layer.}
\label{tab:arch_detection}
\end{table}


==> semantic scene completion/tables/detection_backbone_old.tex <==
\begin{table*}[t!]
\small
\begin{center}
%\vspace{-1.5cm}
\resizebox{\textwidth}{!}{
\label{tab:arch_detection}

\begin{tabular}{|c|c|c|c|c|}
\hline
Layer name & Input                          & Type & Output size  & Layer params                 \\ \hline
sa1\_0     & location of point        & SA   & (2048, 3+128) & (2048, 0.2, {[}64,64,128{]})   \\
sa1\_1     & semantic of point & SA   & (2048, 3+128) & (2048, 0.2, {[}64,64,128{]})   \\
sa\_2      & sa1\_0 + sa1\_1                & SA   & (1024, 3+256) & (1024, 0.4, {[}128,128,256{]}) \\
sa\_3      & sa\_2                          & SA   & (512, 3+256)  & (512, 0.8, {[}128,128,256{]})  \\
sa\_4      & sa\_3                          & SA   & (256, 3+256)  & (256, 1.2, {[}128,128,256{]})  \\
fp\_1      & sa3, sa4                        & FP   & (512, 3+256)  & {[}256, 256{]}                \\
fp\_2      & sa2, sa3                        & FP   & (1024, 3+256) & {[}256, 256{]}                \\ \hline
offset\_1  & fp\_2                          & CBR  & （1024, 256)   & (256, 256, 1)                  \\
offset\_2  & offset\_1                      & CBR  & (1024, 256)   & (256, 256, 1)                  \\
offset\_3  & offset\_2                      & Conv & (1024, 3+256) & (256, 256, 1)                  \\ \hline
proposal\_1       & offset\_3                      & CBR  & (256, 128)    & （128, 128, 1）                  \\
proposal\_2       & conv\_1                        & CBR  & (256, 128)    & (128, 128, 1)                  \\
proposal\_3       & conv\_2                        & Conv & (256, 62)     & (128, 62, 1)                   \\ \hline
\end{tabular}
}
\end{center}
\caption{Parameter details of instance completion stage's detection backbone.FA and FP are set abstraction (SA) layer and feature propagation (FP) layer,respectively. CBR denotes a convolution block consists of a convolution layer flowed by a batchnorm layer and Relu function while Conv means a single a convolution layer.}
\vspace{0.5cm}
\end{table*}


==> semantic scene completion/tables/resNYU.tex <==
\begin{table*}[ht]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l| c |c c c|c c c c c c c c c c c | c|} 
\hline
%   & \multicolumn{3}{c|}{scene completion} & \multicolumn{12}{c}{semantic scene completion} \\ \hline
% Methods  & prec. & recall & IoU & \cellcolor{rgb1}ceil. & \cellcolor{rgb2}floor & \cellcolor{rgb3}wall & \cellcolor{rgb4}win. & \cellcolor{rgb5}chair & \cellcolor{rgb6}bed & \cellcolor{rgb7}sofa & \cellcolor{rgb8}table & \cellcolor{rgb9}tvs & \cellcolor{rgb10}furn. & \cellcolor{rgb11}objs. & avg. \\ 
 & & \multicolumn{3}{c|}{Scene Completion (SC)} & \multicolumn{12}{c|}{Semantic Scene Completion (SSC)} \\ \hline
Methods  & Resolution & prec. & recall & IoU & ceil. & floor & wall & win. & chair & bed & sofa & table & tvs & furn. & objs. & avg. \\ 
\hline
%Lin \etal~\cite{lin2013holistic}  & $(240, 60)$ & 58.5 & 49.9 & 36.4 &  0.0 & 11.7 & 13.3 & 14.1 &  9.4 & 29.0 & 24.0 &  6.0 &  7.0 & 16.2 &  1.1 & 12.0\\
%Geiger \etal~\cite{geiger2015joint} & $(240, 60)$ & 65.7 & 58.0 & 44.4 & 10.2 & 62.5 & 19.1 &  5.8 &  8.5 & 40.6 & 27.7 &  7.0 &  6.0 & 22.6 &  5.9 & 19.6\\ 
% \hline
SSCNet~\cite{song2017semantic-sscnet} & $(240, 60)$ & 57.0 & \textbf{94.5} & 55.1 & 15.1 & 94.7 & 24.4 &  0.0 & 12.6 & 32.1 & 35.0 & 13.0 &  7.8 & 27.1 & 10.1 & 24.7\\
ESSCNet~\cite{zhang2018efficient-esscnet} & $(240, 60)$ & 71.9 & 71.9 & 56.2 & 17.5 & 75.4 & 25.8 &  6.7 & 15.3 & 53.8 & 42.4 & 11.2 &    0 & 33.4 & 11.8 & 26.7\\ 
% VVNet~\cite{guo2018_VVNet}  & 69.8 & 83.1 & 61.1 & 19.3 & {\bfseries 94.8} & 28.0 & 12.2 & 19.6 & {\bfseries 57.0} & {\bfseries 50.5} & {\bfseries 17.6} & 11.9 & 35.6 & 15.3 & 32.9\\ 
% \hline
DDRNet~\cite{li2019rgbd-ddrnet} & $(60, 60)$ & 71.5  & 80.8 & 61.0 & 21.1 & 92.2 & 33.5 & 6.8 & 14.8 & 48.3 & 42.3 & 13.2 & 13.9 & 35.3 &  13.2 & 30.4\\ 
VVNetR-120~\cite{guo2018view-vvnet}  & $(120, 60)$ & 69.8 & 83.1 & 61.1 & 19.3 & 94.8 & 28.0 & 12.2 & 19.6 & 57.0 & 50.5 & 17.6 & 11.9 & 35.6 & 15.3 & 32.9  \\
AICNet~\cite{Li2020aicnet} &$(60, 60)$& 62.4 & 91.8 & 59.2 & 23.2 & 90.8 &32.3& 14.8& 18.2& 51.1& 44.8& 15.2& 22.4& 38.3& 15.7& 33.3\\
TS3D~\cite{garbade2018two-ts3d} & $(240, 60)$ &  - & - & 60.0 & 9.7 & 93.4 & 25.5 & 21.0 & 17.4 & 55.9 & 49.2 & 17.0 & 27.5 & 39.4 & 19.3 & 34.1\\
SATNet~\cite{liu2018see-satnet} & $(60, 60)$ & 67.3 & 85.8 & 60.6 & 17.3 & 92.1 & 28.0 & 16.6 & 19.3 & 57.5 & 53.8 & 17.2 & 18.5 & 38.4 & 18.9 & 34.4 \\
ForkNet~\cite{wang2019forknet}  & $(80, 80)$ & - & - & 63.4 & 36.2 & 93.8 & 29.2 & 18.9 & 17.7 & 61.6 & 52.9 & 23.3 & 19.5 & 45.4 & 20.0 & 37.1 \\
CCPNet~\cite{zhang2019cascaded-ccpnet} & $(240, 240)$ & 74.2  & 90.8 & 63.5 & 23.5 & \textbf{96.3} & 35.7 & 20.2 & 25.8 & 61.4 & 56.1 & 18.1 & 28.1 & 37.8 & 20.1 & 38.5\\ 
Sketch~\cite{Chen_2020_SketchAwareSSC} & $(60, 60)$ & 85.0 & 81.6 & 71.3 & 43.1 & 93.6 & 40.5 & 24.3 & 30.0 & 57.1 & 49.3 & 29.2 & 14.3 & 42.5 & 28.6 & 41.1 \\ 
\hline
\hline
Baseline (BiSeNet) &$(60, 60)$ & 87.6&	78.9& 71.0&
46.9&	93.3&	41.3&	26.7&	30.8&	58.4&	49.5&	27.2&	22.1&	42.2&	28.7&	42.5\\
Ours (BiSeNet) & $(60, 60)$ & 	
%\textbf{91.1}&	82.5&\textbf{76.4}&	\textbf{52.5}&	93.6&	\textbf{50.7}&	\textbf{35.4}&	\textbf{37.3}&	\textbf{62.8}&	\textbf{54.1}&	\textbf{34.0}&	\textbf{22.2}&	\textbf{48.7}&	\textbf{33.8}&	\textbf{47.7}\\
%Ours (BiSeNet) & $(60, 60)$ &  
\textbf{90.7}&	84.6&	\textbf{77.8}& \textbf{53.9}&	93.2&	\textbf{51.3}&	\textbf{38.0}&	\textbf{38.7}&	\textbf{65.0}&	\textbf{56.3}&	\textbf{37.8}&	\textbf{25.9}&	\textbf{51.3}&	\textbf{36.0}&	\textbf{49.8}\\ 
\hline
Baseline (DeepLabv3) &$(60, 60)$ &88.7&	77.7& 70.8&	46.8&	93.4&	42.0&	32.4&	36.0&	61.1&	55.8&	28.2&	27.6&	45.7&	32.9&	45.6\\
Ours (DeepLabv3) & $(60, 60)$ & 	
%\textcolor{blue}{\textbf{91.8}}&	82.6&	\textcolor{blue}{\textbf{76.9}}&	\textcolor{blue}{\textbf{53.0}}&	93.4&	\textcolor{blue}{\textbf{51.8}}&	\textcolor{blue}{\textbf{40.5}}&	\textcolor{blue}{\textbf{43.5}}&	\textcolor{blue}{\textbf{65.1}}&	\textcolor{blue}{\textbf{59.9}}&	\textcolor{blue}{\textbf{34.3}}&	\textcolor{blue}{\textbf{27.9}}&	\textcolor{blue}{\textbf{51.8}}&	\textcolor{blue}{\textbf{38.5}}&	\textcolor{blue}{\textbf{50.9}}\\
\textcolor{blue}{\textbf{92.1}}&	\textcolor{blue}{83.8} &	\textcolor{blue}{\textbf{78.2}} & \textcolor{blue}{\textbf{54.7}} &	\textcolor{blue}{93.8} &	\textcolor{blue}{\textbf{53.2}}&	\textcolor{blue}{\textbf{41.9}}&	\textcolor{blue}{\textbf{43.6}}&	\textcolor{blue}{\textbf{66.2}}&	\textcolor{blue}{\textbf{61.4}}&	\textcolor{blue}{\textbf{38.1}}&	\textcolor{blue}{\textbf{29.8}}&	\textcolor{blue}{\textbf{53.9}}&	\textcolor{blue}{\textbf{40.3}}&	\textcolor{blue}{\textbf{52.4}} \\ 
\hline
\end{tabular}
}
% \vspace{-0.6cm}
\end{center}
\vspace{-0.2cm}
%\caption{\textbf{Results on NYU dataset}. Bold numbers represent the best scores. \textit{Resolution(a, b)} means the input and output resolution is $(a \times 0.6a \times a)$ and the output resolution is $(b \times 0.6b \times b)$.}
\caption{\textbf{Results on NYU dataset}. Bold numbers represent the best scores. \textit{(a, b)} means the input and output resolution.}
\label{tab:SotaOnNYU}
\vspace{-0.3cm}
\end{table*}

==> semantic scene completion/tables/resNYUCAD.tex <==
\begin{table*}[ht]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l| c |c c c|c c c c c c c c c c c | c|} 
\hline
%   & \multicolumn{3}{c|}{scene completion} & \multicolumn{12}{c}{semantic scene completion} \\ \hline
% Methods  & prec. & recall & IoU & \cellcolor{rgb1}ceil. & \cellcolor{rgb2}floor & \cellcolor{rgb3}wall & \cellcolor{rgb4}win. & \cellcolor{rgb5}chair & \cellcolor{rgb6}bed & \cellcolor{rgb7}sofa & \cellcolor{rgb8}table & \cellcolor{rgb9}tvs & \cellcolor{rgb10}furn. & \cellcolor{rgb11}objs. & avg. \\ 
 & & \multicolumn{3}{c|}{Scene Completion (SC)} & \multicolumn{12}{c|}{Semantic Scene Completion (SSC)} \\ \hline
Methods  & Resolution & prec. & recall & IoU & ceil. & floor & wall & win. & chair & bed & sofa & table & tvs & furn. & objs. & avg. \\ 
\hline
%Zheng \etal~\cite{zheng2013beyond} & $(240, 60)$ & 60.1 & 46.7 & 34.6 & - & - & - & - & - & - & - & - & - & - & - & - \\ 
% \hline
%Firman \etal~\cite{firman2016structured} & $(240, 60)$ & 66.5 & 69.7 & 50.8 & - & - & - & - & - & - & - & - & - & - & - & - \\ 
% \hline
SSCNet~\cite{song2017semantic-sscnet} & $(240, 60)$ & 75.4 & \textbf{96.3} & 73.2 & 32.5 & 92.6 & 40.2 &  8.9 & 33.9 & 57.0 & 59.5 & 28.3 &  8.1 & 44.8 & 25.1 & 40.0\\ 
%VVNetR-120~\cite{guo2018view-vvnet} & $(120, 60)$ & 86.4 & 92.0 & 80.3 & - & - & - & - & - & - & - & - & - & - & - & - \\
DDRNet~\cite{li2019rgbd-ddrnet} & $(60, 60)$	& 88.7 & 88.5 & 79.4 & 54.1 & 91.5 & 56.4 & 14.9 & 37.0 & 55.7 & 51.0 & 28.8 & 9.2 & 44.1 & 27.8 & 42.8 \\
AICNet~\cite{Li2020aicnet} &$(60, 60)$& 88.2& 90.3& 80.5& 53.0 &91.2 &57.2& 20.2& 44.6& 58.4& 56.2& 36.2& 9.7& 47.1& 30.4& 45.8\\
TS3D~\cite{garbade2018two-ts3d} & $(240, 60)$   & - & - & 76.1 & 25.9 & 93.8 & 48.9 & 33.4 & 31.2 & 66.1 & 56.4 & 31.6 & 38.5 & 51.4 & 30.8 & 46.2 \\ 
CCPNet~\cite{zhang2019cascaded-ccpnet} & $(240, 240)$ & 91.3 & 92.6 & 82.4 & 56.2 & \textbf{94.6} & 58.7 & 35.1 & 44.8 & 68.6 & 65.3 & 37.6 & 35.5 & 53.1 & 35.2 & 53.2 \\
Sketch~\cite{Chen_2020_SketchAwareSSC} & $(60, 60)$ & 90.6 & 92.2 & 84.2 & 59.7 & 94.3 & 64.3 & 32.6 & 51.7 & 72.0 & \textbf{68.7} & 45.9 & 19.0 & 60.5 & 38.5 &  55.2 \\ 
\hline
\hline
Baseline (BiSeNet) & $(60, 60)$ & 
92.3&	89.0&   82.8 &61.5&	94.2&	62.7&	38.0&	48.1&	69.5&	59.3&	40.1&	25.8&	54.6&	35.3&	53.6\\
Ours (BiSeNet) & $(60, 60)$ & 
%\textbf{93.4}&	90.5&	\textbf{85.1}&	\textbf{63.8}&	94.4&	\textbf{65.1}&	\textbf{43.0}&	\textbf{54.1}&	\textbf{73.9}&	64.7&	\textbf{47.8}&	\textbf{30.4}&	60.2&	\textbf{40.6}&	\textbf{58.0}\\
\textbf{94.2}&	91.3&	\textbf{86.5}&	\textbf{65.6}&	94.4&	\textbf{67.1}&	\textbf{45.2}&	\textbf{57.2}&	\textbf{75.5}&	66.4&	\textbf{50.9}&	\textbf{31.1}&	\textbf{62.5}&	\textbf{42.9}&	\textbf{59.9}\\
\hline
Baseline (DeepLabv3) & $(60, 60)$ & 92.0&	89.3&	82.8 &62.0&	94.1&	63.3&	43.5&	50.8&	73.3&	63.5&	42.2&	40.6&	58.2&	39.7&	57.4\\
Ours (DeepLabv3) & $(60, 60)$ & 
%\textcolor{blue}{\textbf{94.1}}&	90.1&	\textcolor{blue}{\textbf{85.3}}&	\textcolor{blue}{\textbf{63.0}}&	94.2&	\textcolor{blue}{\textbf{67.2}}&	\textcolor{blue}{\textbf{51.4}}&	\textcolor{blue}{\textbf{57.8}}&	\textcolor{blue}{\textbf{77.1}}&	\textcolor{blue}{\textbf{69.3}}&	\textcolor{blue}{\textbf{49.3}}&	\textcolor{blue}{\textbf{44.7}}&	\textcolor{blue}{\textbf{64.1}}&	\textcolor{blue}{\textbf{46.5}}&	\textcolor{blue}{\textbf{62.2}}\\
\textcolor{blue}{\textbf{94.1}}& \textcolor{blue}{91.2}& \textcolor{blue}{\textbf{86.3}} & \textcolor{blue}{\textbf{63.4}}& \textcolor{blue}{94.4}& \textcolor{blue}{\textbf{67.2}}& \textcolor{blue}{\textbf{52.4}}& \textcolor{blue}{\textbf{59.2}}& \textcolor{blue}{\textbf{77.9}}& \textcolor{blue}{\textbf{71.1}}& \textcolor{blue}{\textbf{51.8}}& \textcolor{blue}{\textbf{46.2}}& \textcolor{blue}{\textbf{65.8}}& \textcolor{blue}{\textbf{48.8}}& \textcolor{blue}{\textbf{63.5}}\\
\hline
\end{tabular}
}
% \vspace{-0.6cm}
\end{center}
\vspace{-0.2cm}
%\caption{\textbf{Results on NYUCAD dataset}. Bold numbers represent the best scores. \textit{Resolution(a, b)} means the input resolution is $(a \times 0.6a \times a)$ and the output resolution is $(b \times 0.6b \times b)$.}
\caption{\textbf{Results on NYUCAD dataset}. Bold numbers represent the best scores. \textit{(a, b)} means the input and output resolution.}
\label{tab:SotaOnNYUCAD}
\vspace{-0.3cm}
\end{table*}

==> semantic scene completion/tables/resSUNCG.tex <==
\begin{table*}[t!]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l| c |c c c|c c c c c c c c c c c | c|} 
\hline
  & & \multicolumn{3}{c|}{Scene Completion (SC)} & \multicolumn{12}{c|}{Semantic Scene Completion (SSC)} \\ \hline
Methods  & Resolution 
& prec. & recall & IoU & ceil. & floor & wall & win. & chair & bed & sofa & table & tvs & furn. & objs. & avg. \\ 
\hline

SATNet~\cite{liu2018see-satnet}& $(60, 60)$
& -- & -- & -- & 60.6 & 57.3 & 53.2 & 52.7 & 27.4 & 46.8 & 53.3 & 28.6 & 41.1 & 44.1 & 29.0 & 44.9\\
Sketch~\cite{Chen_2020_SketchAwareSSC}& $(60, 60)$ 
%& SUNCG-RGBD  
& 	\textbf{94.1}&	86.2& 81.8& 77.9&	82.3&	68.4&	57.9&	35.7&	71.8&	63.7&	45.1&	12.8&	64.2&	32.0&	55.6\\
\hline
\hline
Baseline (BiSeNet) & $(60, 60)$ & 90.6&	94.5& 86.0&	71.0&	86.6&	78.4&	78.7&	53.2&	77.4&	77.3&	60.6&	76.4&	83.7&	60.0&	73.0\\

% +\textit{S-I-S Once} & $(60, 60)$ & 92.2&	\textbf{95.5}& \textbf{88.4}&	\textbf{79.3}&	\textbf{88.8}&	\textbf{82.5}&	\textbf{80.4}&	\textbf{56.8}&	\textbf{81.2}&	\textbf{79.5}&	\textbf{63.8}&	\textbf{77.9}&	\textbf{85.3}&	\textbf{67.1}&	\textbf{76.6}\\
%+\textit{S-I-S Once} & $(60, 60)$ & 92.2&	95.5& 88.4&	79.3 &	88.8&	82.5&	80.4&	56.8& 81.2&	 79.5&	63.8& 77.9&	85.3& 67.1 & 76.6\\

Ours (BiSeNet) & $(60, 60)$   &
93.3&	\textbf{96.1}&	\textbf{89.9}&	\textbf{85.2}&	\textbf{90.0}&	\textbf{83.7}&	\textbf{80.8}&	\textbf{60.0}&	\textbf{83.5}&	\textbf{80.9}&	\textbf{68.6}&	\textbf{77.3}&	\textbf{86.7}&	\textbf{70.1}&	\textbf{78.8}\\
\hline
Baseline (DeepLabv3) & $(60, 60)$ & 90.1&	94.5&85.6&70.5&	86.2&	77.5&	79.0&	55.5&	82.8&	78.8&	62.4&	69.5&	81.7&	57.8&	72.9\\
% +\textit{S-I-S Once} &  $(60,60)$  & 91.6 &	95.7 &87.9	&	79.8&	89.5&	81.4&	80.5&	62.0&	84.9&	81.2&	67.7&	72.4&	84.2&	66.9&	77.3\\
Ours (DeepLabv3) & $(60, 60)$ &\textcolor{blue}{92.6} &\textcolor{blue}{\textbf{96.3}} &\textcolor{blue}{\textbf{89.3}}&\textcolor{blue}{\textbf{85.4}} &\textcolor{blue}{\textbf{90.6}} &\textcolor{blue}{\textbf{82.6}} &\textcolor{blue}{\textbf{80.9}} &\textcolor{blue}{\textbf{62.9}} &\textcolor{blue}{\textbf{84.5}} & \textcolor{blue}{\textbf{82.6}}&\textcolor{blue}{\textbf{71.6}} &\textcolor{blue}{\textbf{72.6}} &\textcolor{blue}{\textbf{85.6}}&\textcolor{blue}{\textbf{69.7}} & \textcolor{blue}{\textbf{79.0}}\\
% Ours (DeepLabv3) & $(60, 60)$& 
% 91.6&	\textcolor{blue}{\textbf{95.7}}&  \textcolor{blue}{\textbf{87.9}}& \textcolor{blue}{\textbf{79.8}}& \textcolor{blue}{\textbf{89.5}}& 	\textcolor{blue}{\textbf{81.4}}& 	\textcolor{blue}{\textbf{80.5}}& 	\textcolor{blue}{\textbf{62.0}}& 	\textcolor{blue}{\textbf{84.9}}& 	\textcolor{blue}{\textbf{81.2}}& 	\textcolor{blue}{\textbf{67.7}}& 	\textcolor{blue}{\textbf{72.4}}& 	\textcolor{blue}{\textbf{84.2}}& 	\textcolor{blue}{\textbf{66.9}}& 	\textcolor{blue}{\textbf{77.3}}\\
\hline
\end{tabular}
}
\end{center}
\vspace{-0.2cm}
%\caption{\textbf{Results on SUNCG-RGBD dataset}. Bold numbers represent the best scores. \textit{Resolution(a, b)} means the input resolution is $(a \times 0.6a \times a)$ and the output resolution is $(b \times 0.6b \times b)$.}
\caption{\textbf{Results on SUNCG-RGBD dataset}. Bold numbers represent the best scores. \textit{(a, b)} means the input and output resolution.}
\label{tab:SotaOnSUNCG}
\vspace{-0.6cm}
\end{table*}


==> tables/GRNet.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[t!]
% \small
% \begin{center}
% %\vspace{-4.5cm}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|cccc|}
% \hline
%                                             & Layer name     & Input                           & Output size    \\ \hline                & Layer params                  \\ \hline
                                            
% \multirow{3}{*}{Semantic Encoder}           & FC\_1          & Semantic Vector                  & (16, 1)         \\   %              & (8,16)                        \\
%                                             & FC\_2          & FC\_1                           & (64, 1)           \\  %            & (16,64)                       \\
%                                             & Reshape\_1     & FC\_2                           & (1, $4^{3}$)    \\\hline%   &  -                             \\ \hline
% \multirow{6}{*}{Geometry Encoder}           & Griding        & Partial Point Cloud             & (1, $32^{3}$)   \\%   &   -                            \\
%                                             & Conv3D\_1      & 3D Grid                         & (16, $16^{3}$)  \\%  & (16, $4^{3}$) \\
%                                             & Conv3D\_2      & Conv3D\_1                       & (32, $8^{3}$)   \\%  & (32, $4^{3}$) \\
%                                             & Conv3D\_3      & Conv3D\_2                       & (32, $4^{3}$)   \\%  & (32, $4^{3}$) \\ 

%                                             & Concat\_1      & Conv3D\_3, Reshape\_1                 & (33, $4^{3}$) \\% &  -                             \\
%                                             & Conv3D\_4      & Concat\_1                       & (32, $4^{3}$)  & \\ \hline  %(1, $1^{3}$)  \\ \hline 
%  \multirow{3}{*}{Decoder}                                             & Deconv3D\_1    & Conv3D\_4             & (32, $8^{3}$)  \\ %& (32, $4^{3}$) \\
%                                             & Deconv3D\_2    & Concat(Deconv3D\_1, Conv3D\_2)          & (16, $16^{3}$) \\ %& (16, $4^{3}$) \\
%                                             & Deconv3D\_3    & Concat(Deconv3D\_2, Conv3D\_1)          & (1, $32^{3}$)  \\ \hline%& (1, $4^{3}$)  \\ \hline
% \multirow{5}{*}{Feature-Point 
%                 downsampling(ds)}               & Re-Griding     & Deconv3D\_1                     & (1, $32^{3}$)      \\  %       &   -       \\
%                                             & Point\_ds      & Re-Griding, Partical Point Cloud & (3, 1024)              \\  %        &   -                            \\
%                                             & Feature\_ds\_1 & ConCat(Point\_ds, Conv3D\_2)             & (128, 1024)     \\ %               &   -                            \\ %\cline{2-5} 
%                                             & Feature\_ds\_2 & ConCat(Point\_ds, Conv3D\_1)            & (256, 1024)      \\  %              &   -                            \\
%                                             & Concat\_2      & Feature\_DS\_1, Feature\_DS\_2     & (384, 1024)            \\ \hline %       &   -                            \\ \hline
% \multirow{4}{*}{MLP}                        & FC\_3          & Concat\_2                       & (96, 1024)                \\ %     & (384, 96)                      \\
%                                             & FC\_4          & FC\_3                           & (24, 1024)               \\ %      & (96, 24)                       \\
%                                             %& Tile\_1        & Point\_ds)                      & (3, 8192)                       &   -                   \\ %\hline
%                                             & Reshape\_2     & FC\_4                           & (3, 8192)                \\ %       &   -                           \\ %\hline
%                                             & Output         & Tile(Point\_ds)+Reshape\_2      & (3, 8192)                \\ \hline      &   -                           \\ \hline
% \end{tabular}
% }

% \end{center}
% %\vsapce{0.2cm}
% \caption{Parameter details of shape reconstruction module.Tile means a operation that replicate the input $(3,m)$ $n$ times and return a new point set with the size of $(3,mn)$.}
% \label{tab:arch_grnet}
% \end{table*}
%\multirow{2}{*}{}  

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
                                                                                       & Layer name     & Input                           & Output size                    \\ \hline
\multirow{3}{*}{Semantic Encoder}                                                      & FC\_1          & Semantic Vector                 & (16,1)                         \\
                                                                                       & FC\_2          & FC\_1                           & (64,1)                         \\
                                                                                       & Reshape\_1     & FC\_2                           & (1, $4^{3}$)   \\ \hline
\multirow{6}{*}{Geometry Encoder}                                                      & Griding        & Partial Point Cloud             & (1, $32^{3}$) \\
                                                                                       & Conv3D\_1      & Griding                         & (16, $16^{3}$)                      \\
                                                                                       & Conv3D\_2      & Conv3D\_1                       & (32, $8^{3}$)                     \\
                                                                                       & Conv3D\_3      & Conv3D\_2                       & (32, $4^{3}$)                     \\
                                                                                       & Concat\_1      & Conv3D\_3, FC\_2                 & (33, $4^{3}$)  \\
                                                                                       & Conv3D\_4      & Concat\_1                       & (32, $4^{3}$)  \\ \hline
\multirow{3}{*}{Decoder}                                                               & Deconv3D\_1    & Conv3D\_4                       & (32, $8^{3}$) \\
                                                                                       & Deconv3D\_2    & Deconv3D\_1, Conv3D\_2           & (32, $16^{3}$) \\
                                                                                       & Deconv3D\_3    & Deconv3D\_2, Conv3D\_1           & (32, $32^{3}$)  \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Feature-Point\\  DownSampling(DS)\end{tabular}} & Rev-Griding     & Deconv3D\_3                     & (1, $32^{3}$)   \\
                                                                                       & Point\_DS      & Rev-Griding, Partial Point Cloud & (3,1024)                       \\
                                                                                       & Feature\_DS\_1 & Point\_DS, Conv3D\_2             & (128,1024)                     \\ %\cline{2-4} 
                                                                                       & Feature\_DS\_2 & Point\_DS, Conv3D\_1             & (256,1024)                     \\
                                                                                       & Concat\_2      & Feature\_DS\_1, Feature\_DS\_2   & (384,1024)                     \\ \hline
\multirow{4}{*}{MLP}                                                                   & FC\_3          & Concat\_2                       & (96,1024)                      \\
                                                                                       & FC\_4          & FC\_3                           & (24,1024)                      \\
                                                                                       & Reshape\_2     & FC\_4                           & (3,8192)                       \\ %\hline
                                                                                       & Output         & Tile(Point\_DS), Reshape\_2      & (3, 8192)                \\ \hline 
\end{tabular}
}
\vspace{0.2cm}
\caption{Architecture details of shape completion. Tile denotes a operation that replicate the input $(3,m)$ $n$ times and return a new point set with the size of $(3,m\times n)$. We use the Griding, Rev-Griding and downsampling operations proposed in \cite{xie2020grnet}}
\label{tab:arch_grnet}
\end{table}

==> tables/Scene.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[t!]
% % \vspace{-1.0cm}
% \begin{center}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|ccccc|}
% \hline
%                           & Layer name   & Input                                     & Type & Output size    & Layer params                       \\ \hline
% \multirow{14}{*}{Encoder} & Conv3D\_1\_0 & Semantic Volume $V_S$                        & CBR  & (3,  60,  36,  60)   & (1,  3,  3\textasciicircum{}\{3\})     \\
%                           & Conv3D\_1\_1 & Conv3D\_1\_0                              & CBR  & (64,  60,  36,  60)  & (3,  64,  3\textasciicircum{}\{3\})    \\
%                           & Conv3D\_1\_2 & Conv3D\_1\_1                              & CBR  & (128,  60,  36,  60) & (64,  128,  3\textasciicircum{}\{3\})  \\
%                           & Conv3D\_2\_0 & TSDF Volume $V_T$                            & CBR  & (3,  60,  36,  60)   & \color{red}{(12,  3,  3\textasciicircum{}\{3\})}    \\
%                           & Conv3D\_2\_1 & Conv3D\_2\_0                              & CBR  & (64,  60,  36,  60)  & (3,  64,  3\textasciicircum{}\{3\})    \\
%                           & Conv3D\_2\_2 & Conv3D\_2\_1                              & CBR  & (128,  60,  36,  60) & (64,  128,  3\textasciicircum{}\{3\})  \\ \cline{2-6} 
%                           & DDR\_0       & Conv3D\_1\_2+Conv3D\_2\_2                 & DDR  & (128,  30,  18,  30) & (1,  2)                              \\
%                           & DDR\_1\_1    & DDR\_0                                    & DDR  & (128,  30,  18,  30) & (1,  1)                              \\
%                           & DDR\_1\_2    & DDR\_1\_1                                 & DDR  & (128,  30,  18,  30) & (2,  1)                              \\
%                           & DDR\_1\_3    & DDR\_1\_2                                 & DDR  & (128,  30,  18,  30) & (3,  1)                              \\ \cline{2-6} 
%                           & DDR\_2       & DDR\_1\_3+Down & DDR  & (256,  15,  9,  15)  & (1,  2)                              \\
%                           & DDR\_3\_1    & DDR\_2                                    & DDR  & (256,  15,  9,  15)  & (1,  1)                              \\
%                           & DDR\_3\_2    & DDR\_3\_1                                 & DDR  & (256,  15,  9,  15)  & (2,  1)                              \\
%                           & DDR\_3\_3    & DDR\_3\_2                                 & DDR  & (256,  15,  9,  15)  & (3,  1)                              \\ \hline
% \multirow{3}{*}{Decoder}  & Deconv3D\_1  & DDR\_3\_3 + DDR\_1\_3 + Down              & CBR  & (128,  30,  18,  30) & (256,  128,  3\textasciicircum{}\{3\}) \\
%                           & Deconv3D\_2  & Deconv3D\_1                               & CBR  & (128,  60,  36,  60) & (128,  128,  3\textasciicircum{}\{3\}) \\
%                           & Conv3D\_3    & Deconv3D\_2 + Up                              & Conv     & (12,  60,  36,  60)  & (128,  12,  1\textasciicircum{}\{3\})  \\ \hline
% \end{tabular}
% }
% \end{center}
% \caption{Architecture and parameters details of scene completion stage. $Down$ means the downsampling operation of the combination feature of (Conv3D\_1\_2+Conv3D\_2\_2) while the $Up$ is the upsampling operation on output feature of Deconv3D\_1.CBR denotes a convolution block consists of a convolution layer flowed by a batchnorm layer and Relu function while Conv means a single a convolution layer.For DDR block, the layer params represents the dilation and downsample rate, respectively.}
% \label{tab:arch_scene}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
\small
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|}
\hline
                                                                             & Layer name   & Input                     & Type & Output size    \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Semantic\\ Encoder\end{tabular}}  & Conv3D\_1\_0 & Semantic Volume V_S        & CBR  & (3,60,36,60)   \\
                                                                             & Conv3D\_1\_1 & Conv3D\_1\_0              & CBR  & (64,60,36,60)  \\
                                                                             & Conv3D\_1\_2 & Conv3D\_1\_1              & CBR  & (128,60,36,60) \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Geometry \\ Encoder\end{tabular}} & Conv3D\_2\_0 & TSDF Volume V_T            & CBR  & (3,60,36,60)   \\
                                                                             & Conv3D\_2\_1 & Conv3D\_2\_0              & CBR  & (64,60,36,60)  \\
                                                                             & Conv3D\_2\_2 & Conv3D\_2\_1              & CBR  & (128,60,36,60) \\
                                                                             & Add\_1       & Conv3D\_1\_2, Conv3D\_2\_2 & -     & (128,60,36,60) \\ \hline
\multirow{9}{*}{Encoder}                                                     & DDR\_0       & Add\_1                       & DDR  & (128,30,18,30) \\
                                                                             & DDR\_1       & DDR\_0                    & DDR  & (128,30,18,30) \\
                                                                             & DDR\_2       & DDR\_1                    & DDR  & (128,30,18,30) \\
                                                                             & DDR\_3       & DDR\_2                    & DDR  & (128,30,18,30) \\
                                                                             & Add\_2       & DDR\_3, Down(Add\_1)       & -    & (128,30,18,30) \\ \cline{2-5} 
                                                                             & DDR\_4       & Add\_2                    & DDR  & (256,15,9,15)  \\
                                                                             & DDR\_5       & DDR\_4                    & DDR  & (256,15,9,15)  \\
                                                                             & DDR\_6       & DDR\_5                    & DDR  & (256,15,9,15)  \\
                                                                             & DDR\_7       & DDR\_6                    & DDR  & (256,15,9,15)  \\ \hline
\multirow{4}{*}{Decoder}                                                     & Deconv3D\_1  & DDR\_7                    & DBR  & (128,30,18,30) \\
                                                                             & Add\_3       & Deconv3D\_1, Add\_2        & -    & (128,30,18,30) \\
                                                                             & Deconv3D\_2  & Add\_3                    & DBR  & (128,60,36,60) \\
                                                                             & Conv3D\_3    & Deconv3D\_2, Up(Add\_3)    & Conv & (12,60,36,60)  \\ \hline
\end{tabular}
}
\end{center}
\caption{Architecture and parameters details of scene completion stage. \textit{Down}, \textit{Up} mean downsampling and upsampling operation, respectively. \textit{CBR} denotes a convolution block consists of a $3\times 3$ convolution layer flowed by a batchnorm layer and Relu function and \textit{DBR} replaces the convolution layer of \textit{CBR} with a $4\times 4$ deconvolution layer.  \textit{Conv} means a single  $1\times 1$ convolution layer.}
\label{tab:arch_scene}
\end{table}

==> tables/ablation-detection.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t!]
\tiny
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|ccccccccc|c|}
\hline
Datasets                    & Iteration       & win.          & chair         & bed           & sofa          & table         & tvs           & furn.         & objs.         & avg           \\ \hline
\multirow{3}{*}{NYU}        & I               & 7.5           & 21.1          & 59.6          & 45.7          & 20.1          & 18.0          & 27.6          & 7.4           & 25.6          \\
                            & S0 + Iter I-S   & 15.8          & 30.0          & 66.0          & 48.8          & 29.8          & 31.6          & 35.9          & 19.0          & 34.6          \\
                            & S0 + 2 Iter I-S & \textbf{21.9} & \textbf{33.2} & \textbf{69.0} & \textbf{55.8} & \textbf{43.4} & \textbf{36.3} & \textbf{43.2} & \textbf{23.8} & \textbf{40.8} \\ \hline
\multirow{3}{*}{NYUCAD}     & I               & 32.7          & 38.3          & 64.9          & 54.4          & 43.1          & 35.1          & 38.9          & 21.7          & 41.1          \\
                            & S0 + Iter I-S   & 30.1          & 50.0          & 66.6          & 52.3          & 44.0          & 36.8          & 46.3          & 31.3          & 44.5          \\
                            & S0 + 2 Iter I-S & \textbf{42.0} & \textbf{50.2} & \textbf{72.3} & \textbf{60.5} & \textbf{58.5} & \textbf{46.7} & \textbf{54.3} & \textbf{37.2} & \textbf{52.7} \\ \hline
\multirow{3}{*}{SUNCG-RGBD} & I               & 74.2          & 65.0          & 83.9          & 82.0          & 67.3          & 32.7          & 72.1          & 43.3          & 65.0          \\
                            & S0 + Iter I-S   & 76.1          & 75.7          & 85.2          & \textbf{84.2} & 70.8          & \textbf{35.6} & 82.6          & 53.3          & 70.4          \\
                            & S0 + 2 Iter I-S & \textbf{76.8} & \textbf{76.9} & \textbf{86.6} & 83.2          & \textbf{72.9} & 34.0          & \textbf{86.0} & \textbf{56.5} & \textbf{71.6} \\ \hline
\end{tabular}
}
\end{center}
\caption{Ablation studies of the effects of the scene completion to the proposal generation module of instance completion on three datasets. The numbers reported are detection mAP (IoU=0.25) for different classes, where $I$ is the instance completion and $S$ is the scene completion.}
\label{tab:detection}
\end{table*}

==> tables/detection_backbone.tex <==
% \begin{table}[t!]
% \small
% \begin{center}
% %\vspace{-1.5cm}
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% Layer & Input                          & Type & Output size  & Layer params                 \\ \hline
% $sa1_0$     & location        & \textit{SA}   & (2048, 3+128) & (2048, 0.2, (64,64,128))   \\
% $sa1_1$     & semantic & \textit{SA}   & (2048, 3+128) & (2048, 0.2, (64,64,128))   \\
% sa2      & $sa1_0$ + $sa1_1$                & \textit{SA}   & (1024, 3+256) & (1024, 0.4, (128,128,256)) \\
% sa3      & sa2                          & \textit{SA}   & (512, 3+256)  & (512, 0.8, (128,128,256))  \\
% sa4      & sa3                          & \textit{SA}   & (256, 3+256)  & (256, 1.2, (128,128,256))  \\
% fp1      & sa3, sa4                        & \textit{FP}   & (512, 3+256)  &(256, 256)               \\
% fp2      & sa2, sa3                        & \textit{FP}   & (1024, 3+256) & (256, 256)              \\ \hline
% offset\_1  & fp\_2                          & \textit{CBR}  & 1024, 256)   & (256, 256, 1                  \\
% offset\_2  & offset\_1                      & \textit{CBR}  & 1024, 256)   & (256, 256, 1)                 \\
% offset\_3  & offset\_2                      & \textit{Conv} & 1024, 3+256) & (256, 256, 1)                  \\ \hline
% proposal\_1       & offset\_3                      & \textit{CBR}  & (256, 128)    & 128, 128, 1                  \\
% proposal\_2       & conv\_1                        & \textit{CBR}  & (256, 128)    & (128, 128, 1)                  \\
% proposal\_3       & conv\_2                        & \textit{Conv} & (256, 62)     & (128, 62, 1)                   \\ \hline
% \end{tabular}
% }
% % \vspace{0.5cm}
% \end{center}
% \caption{Architecture details of proposal generation. \textit{SA} and \textit{FP} represent set abstraction layer and feature propagation layer, respectively. \textit{CBR} denotes a convolution block consists of a convolution layer followed by a batchnorm and Relu function while \textit{Conv} means a single a convolution layer.}
% \label{tab:arch_detection}
% \end{table}

\begin{table}[]
\begin{center}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
Layer name  & Input                          & Type & Output size  \\ \hline
sa\_1\_0      & location of point cloud        & SA   & (2048, 3+128) \\
sa\_1\_1     & semantic vector of point cloud & SA   & (2048, 3+128) \\
sa\_2       & sa\_1\_0, sa\_1\_1             & SA   & (1024,3+256) \\
sa\_3       & sa\_2                          & SA   & (512, 3+256)  \\
sa\_4       & sa\_3                          & SA   & (256, 3+256)  \\
fp\_1       & sa\_3, sa\_4                        & FP   & (512, 3+256)  \\
fp\_2       & sa\_2, sa\_3                        & FP   & (1024, 3+256) \\ \hline
offset\_1   & fp\_2                          & CBR  & （1024, 256)   \\
offset\_2   & offset\_1                      & CBR  & (1024, 256)   \\
offset\_3   & offset\_2                      & Conv & (1024, 3+256) \\ \hline
proposal\_1 & offset\_3                      & CBR  & (256, 128)    \\
proposal\_2 & proposal\_1                        & CBR  & (256, 128）    \\
proposal\_3 & proposal\_2                        & Conv & (256, 62)     \\ \hline
\end{tabular}
}
\end{center}
\caption{Architecture details of proposal generation. \textit{SA} and \textit{FP} represent the set abstraction layer and feature propagation layer, respectively. \textit{CBR} denotes a convolution block consists of a $1\times 1$ convolution layer followed by a batchnorm and Relu function while \textit{Conv} means a single $1\times 1$ convolution layer.}
\label{tab:arch_detection}
\end{table}


==> tables/detection_backbone_old.tex <==
\begin{table*}[t!]
\small
\begin{center}
%\vspace{-1.5cm}
\resizebox{\textwidth}{!}{
\label{tab:arch_detection}

\begin{tabular}{|c|c|c|c|c|}
\hline
Layer name & Input                          & Type & Output size  & Layer params                 \\ \hline
sa1\_0     & location of point        & SA   & (2048, 3+128) & (2048, 0.2, {[}64,64,128{]})   \\
sa1\_1     & semantic of point & SA   & (2048, 3+128) & (2048, 0.2, {[}64,64,128{]})   \\
sa\_2      & sa1\_0 + sa1\_1                & SA   & (1024, 3+256) & (1024, 0.4, {[}128,128,256{]}) \\
sa\_3      & sa\_2                          & SA   & (512, 3+256)  & (512, 0.8, {[}128,128,256{]})  \\
sa\_4      & sa\_3                          & SA   & (256, 3+256)  & (256, 1.2, {[}128,128,256{]})  \\
fp\_1      & sa3, sa4                        & FP   & (512, 3+256)  & {[}256, 256{]}                \\
fp\_2      & sa2, sa3                        & FP   & (1024, 3+256) & {[}256, 256{]}                \\ \hline
offset\_1  & fp\_2                          & CBR  & （1024, 256)   & (256, 256, 1)                  \\
offset\_2  & offset\_1                      & CBR  & (1024, 256)   & (256, 256, 1)                  \\
offset\_3  & offset\_2                      & Conv & (1024, 3+256) & (256, 256, 1)                  \\ \hline
proposal\_1       & offset\_3                      & CBR  & (256, 128)    & （128, 128, 1）                  \\
proposal\_2       & conv\_1                        & CBR  & (256, 128)    & (128, 128, 1)                  \\
proposal\_3       & conv\_2                        & Conv & (256, 62)     & (128, 62, 1)                   \\ \hline
\end{tabular}
}
\end{center}
\caption{Parameter details of instance completion stage's detection backbone.FA and FP are set abstraction (SA) layer and feature propagation (FP) layer,respectively. CBR denotes a convolution block consists of a convolution layer flowed by a batchnorm layer and Relu function while Conv means a single a convolution layer.}
\vspace{0.5cm}
\end{table*}

